HADRON: Human-friendly Control and Artificial Intelligence for Military Drone Operations

As drones are getting more and more entangled in our society, more untrained users require the capability to operate them. This scenario is to be achieved through the development of artificial intelligence capabilities assisting the human operator in controlling the Unmanned Aerial System (UAS) and processing the sensor data, thereby alleviating the need for extensive operator training. This paper presents the HADRON project that seeks to develop and test multiple novel technologies to enable human-friendly control of drone swarms. This project is divided into three main parts. The first part consists of the integration of different technologies for the intuitive control of drones, focusing on novice or inexperienced pilots and operators. The second part focuses on the development of a multi-drone system that will be controlled from a command and control station, in which an expert pilot can supervise the operations of the multiple drones. The third part of the project will focus on reducing the cognitive load on human operators, whether they are novice or expert pilots. For this, we will develop AI tools that will assist drone operators with semi-automated real-time data processing.

==> resources/table_functionalities.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[bth]
\centering
\begin{tabular}{|c|cl|}
\hline
\textbf{Module}                                                                                          & \multicolumn{2}{c|}{\textbf{Functionality}}                                                                                                                                                             \\ \hline
\multirow{15}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Human-Machine\\ Interface Design\end{tabular}}}      & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Audio Feedback}}}                                          & Drone status updates.                                                                          \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Mission status updates.                                                                        \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Information about environment (e.g. number of detected enemies, localization of target...).    \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Audio Command}}}                                           & Implementation of main drone commands (e.g. take off, land...).                                \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Go to waypoint command.                                                                        \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Implementation of sending pre-programmed missions (e.g. coverage of a certain area).           \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\textbf{Hand Gestures}}                                                            & Implementation of main drone commands (e.g. take off, land, RPY and thrust).                   \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{Tablet Control}}}                                          & Visualization of typical drone status information (e.g. IMU, odometry, position, battery...).  \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Map visualization.                                                                             \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Trajectory designer with waypoints.                                                            \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Mission planner.                                                                               \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\multirow{4}{*}{\textbf{Augmented Reality}}}                                       & Small interface with basic information about the drone status (e.g. battery status, odometry). \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Small interface with map situation of drone.                                                   \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Possibility of changing between drone and pilot vision.                                        \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Basic control of drone with virtual reality controller.                                        \\ \hline
\multirow{6}{*}{\textbf{Multi-Agent System}}                                                             & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Command and \\ Control Interface\end{tabular}}} & Powerful stand-alone capability.                                                               \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Patrolling / Coverage}}}                                   & Deployment of coverage mission for surveillance purposes.                                      \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Possibility of changing drone trajectory for specific task.                                    \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Information about environment (e.g. number of detected enemies, localization of target...).    \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Drone Formations}}}                                        & Follow trajectory while maintaining formation.                                                 \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & Follow me function while maintaining formation.                                                \\ \hline
\multirow{6}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Artificial Intelligence\\ Capabilities\end{tabular}}} & \multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Target Detection}}}                                        & The system has to detect, localize and track people.                                           \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & The system has to detect, localize and track vehicles.                                         \\ \cline{3-3} 
                                                                                                         & \multicolumn{1}{c|}{}                                                                                  & The system has to differentiate between friendly, unknown and enemy.                           \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\textbf{Defect Detection}}                                                         & The system has to detect different types of defects.                                           \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\textbf{Battery   analysis}}                                                       & The system has to estimate the battery consumption required for achieving the mission.         \\ \cline{2-3} 
                                                                                                         & \multicolumn{1}{c|}{\textbf{Image Quality}}                                                            & The system has to assess image quality in case missions have to be repeated for more data.     \\ \hline
\end{tabular}

\caption{Summary of the different functionalities expected from the HADRON project}
\label{tab-func}
\end{table*}
